Teaching Structured Vision&Language Concepts to Vision&Language Models

Vision and Language (VL) models have demonstrated remarkable zero-shot performance in a variety of tasks. However, some aspects of complex language understanding still remain a challenge. We introduce the collective notion of Structured Vision&Language Concepts (SVLC) which includes object attributes, relations, and states which are present in the text and visible in the image. Recent studies have shown that even the best VL models struggle with SVLC. A possible way of fixing this issue is by collecting dedicated datasets for teaching each SVLC type, yet this might be expensive and time-consuming. Instead, we propose a more elegant data-driven approach for enhancing VL models' understanding of SVLCs that makes more effective use of existing VL pre-training datasets and does not require any additional data. While automatic understanding of image structure still remains largely unsolved, language structure is much better modeled and understood, allowing for its effective utilization in teaching VL models. In this paper, we propose various techniques based on language structure understanding that can be used to manipulate the textual part of off-the-shelf paired VL datasets. VL models trained with the updated data exhibit a significant improvement of up to 15% in their SVLC understanding with only a mild degradation in their zero-shot capabilities both when training from scratch or fine-tuning a pre-trained model.

==> sup/sup.tex <==

caption: summer sunny day at the country side - country road
pos:  country road that is summer sunny day at the country side
neg_rb: <start_of_text>summer dirty day at the country side - country road <end_of_text>
neg_model: <start_of_text>summer rainy day at the country side country road <end_of_text>

caption: caucasian wedding couple posing on the yacht .
pos: ie: a couple posing on the yacht
neg_rb: <start_of_text>caucasian wedding couple posing parked on the yacht . <end_of_text>
neg_model: <start_of_text>italian wedding couple posing on the yacht <end_of_text>


caption: little boy playing drums , little drummer .
neg_rb: <start_of_text>teeny boy playing drums , teeny drummer . <end_of_text>
neg_model: <start_of_text>little boy playing a little drummer <end_of_text>

caption: person attends the premiere at amc empire theater
neg_rb: 
neg_model: <start_of_text>person attends the concert at amc empire theater <end_of_text>

caption: a typical violin with flag and bow isolated over a white background
neg_rb: <start_of_text>a typical violin with flag and bow isolated over a fresh background <end_of_text>
neg_model: <start_of_text>a typical violin with flag and stripes isolated over a white background <end_of_text>

caption: aerial shot of kayaks going down a river in the highlands
pos:  a boat that is going down a river in the highlands
neg_rb: 
neg_model: <start_of_text>aerial shot of kayaks going across a river in the highlands <end_of_text>

caption: melting ice cream on the beach
neg_rb: <start_of_text>melting nylon cream on the beach <end_of_text>
neg_model: <start_of_text>melting ice cream at the beach <end_of_text>

caption: the cost of caring many families spend more than half of every dollar they earn to care for the needs of family members with person .
neg_rb: <start_of_text>the cost of caring many families spend more than half of every dollar they earn to care for the needs of family members growing on person . <end_of_text>
neg_model: <start_of_text>the cost of caring many caregivers spend more than half of every dollar they earn to care for the needs of family members with person <end_of_text>

caption: i 'm officially obsessed with this hair style
pos: ive been wearing this hair style for a while now
neg_rb: <start_of_text>i 'm officially obsessed of this hair style <end_of_text>
neg_model: <start_of_text>i m officially obsessed with this retro style <end_of_text>

caption: # shoots the ball against sports team .
neg_rb: <start_of_text># shoots the ball covered in sports team . <end_of_text>
neg_model: <start_of_text>shoots the ball against sportsmanship <end_of_text>

caption: actor attends the opening night .
neg_rb: 
neg_model: <start_of_text>actor attends the opening ... <end_of_text>

caption: view of the doors from the garden room .
neg_rb: <start_of_text>view part of the doors from the garden room . <end_of_text>
neg_model: <start_of_text>out of the doors from the garden room <end_of_text>

caption: fireworks explode ... behind landmark brandenburg gate to usher in the new year .
neg_rb: <start_of_text>fireworks explode ... from landmark brandenburg gate to usher in the new year . <end_of_text>
neg_model: <start_of_text>fireworks explode behind landmark brandenburg gate to usher on the new year <end_of_text>

caption: at the end of the day , a hotel is only as good as its beds .
pos: ughing at the end of the day
neg_rb: <start_of_text>at the end lying on the day , a hotel is only as good as its beds . <end_of_text>
neg_model: <start_of_text>at the end of the day a hotel is only as good as its owners <end_of_text>

caption: watch tv on the verandah or the deck
pos:  watching tv on the verandah or the deck
neg_rb: <start_of_text>watch tv behind the verandah or the deck <end_of_text>
neg_model: <start_of_text>live tv on the verandah or the deck <end_of_text>

caption: fireworks light the sky during new year 's celebrations
neg_rb: <start_of_text>fireworks vast the sky during new year 's celebrations <end_of_text>
neg_model: <start_of_text>fireworks light the sky during new millennium s celebrations <end_of_text>

caption: large deer in a fight in winter
neg_rb: <start_of_text>large deer between a fight between wbetweenter <end_of_text>
neg_model: <start_of_text>large deer losing a fight in winter <end_of_text>

caption: clouds sailing above a city
neg_rb: <start_of_text>clouds sailing covering a city <end_of_text>
neg_model: <start_of_text>clouds soar above a city <end_of_text>

caption: a cheetah pictured at a game reserve
pos:  a cheetah that is pictured at a game reserve
neg_rb: 
neg_model: <start_of_text>a cheetah ball at a game reserve <end_of_text>

caption: actor during an interview with comedian --
neg_rb: <start_of_text>actor during an interview along comedian -- <end_of_text>
neg_model: <start_of_text>actor during an exchange with comedian <end_of_text>

caption: an illustration of a scary sports mascot with claws out
neg_rb: <start_of_text>an illustration of a scary sports mascot above claws out <end_of_text>
neg_model: <start_of_text>an illustration of a scary sports mascot that claws out <end_of_text>

caption: a cute kitten with a bow sits in sneakers .
neg_rb: <start_of_text>a cute kitten with a bow sits watching sneakers . <end_of_text>
neg_model: <start_of_text>a cute cat with a bow sits in sneakers <end_of_text>

caption: a car stranded in flood waters
pos:  a car that is stranded in flood waters
neg_rb: 
neg_model: <start_of_text>a fisherman stranded in flood waters <end_of_text>


caption: person of musical group performs at festival
pos:  a person performing at festival
neg_rb: <start_of_text>person playing musical group performs at festival <end_of_text>
neg_model: <start_of_text>person of musical group pictured at festival <end_of_text>

caption: colorful squatter shacks and houses
pos:  a squatter house and a squatter shack
neg_rb: 
neg_model: <start_of_text>colorful wooden shacks and houses <end_of_text>

caption: statesman plays a game of football with year pupils today
pos: erstwhile football player played by year pupils today
neg_rb: <start_of_text>statesman plays a game of football looking at year pupils today <end_of_text>
neg_model: <start_of_text>statesman plays a game of football sixth year pupils today <end_of_text>

caption: studio portrait of young girl standing and holding a fan
pos:  a girl standing and holding a fan
neg_rb: 
neg_model: <start_of_text>studio portrait of young girl standing and holding a candle <end_of_text>

caption: black girl in white sneakers on the sand of beach
pos:  a girl in black sneakers on the sand of beach
neg_rb: <start_of_text>black girl in different sneakers on the sand of beach <end_of_text>
neg_model: <start_of_text>black girl in white sneakers on the sands of beach <end_of_text>


